Robust Resource Allocation Using Edge Computing for Vehicle to Infrastructure (V2I) Networks

Development of autonomous and self-driving vehicles requires agile and reliable services to manage hazardous road situations. Vehicular Network is the medium that can provide high-quality services for self-driving vehicles. The majority of service requests in Vehicular Networks are delay intolerant (e.g., hazard alerts, lane change warning) and require immediate service. Therefore, Vehicular Networks, and particularly, Vehicle-to-Infrastructure (V2I) systems must provide a consistent real-time response to autonomous vehicles. During peak hours or disasters, when a surge of requests arrives at a Base Station, it is challenging for the V2I system to maintain its performance, which can lead to hazardous consequences. Hence, the goal of this research is to develop a V2I system that is robust against uncertain request arrivals. To achieve this goal, we propose to dynamically allocate service requests among Base Stations. We develop an uncertainty-aware resource allocation method for the federated environment that assigns arriving requests to a Base Station so that the likelihood of completing it on-time is maximized. We evaluate the system under various workload conditions and oversubscription levels. Simulation results show that edge federation can improve robustness of the V2I system by reducing the overall service miss rate by up to 45%.

==> NEW PAPER LATEX/Sources/approach.tex <==
\section{Robust V2I System based on Federated Base Stations}\label{sec:approach}
\subsection{Federation-Enabled Base Station}
To enable the robustness against uncertainty in task request arrival of a V2I system, we propose to federate \bs s in a dynamic manner. Thus, \bs s can augment the computational power upon demand and keep the Quality of Service (QoS), even if faced with oversubscription. Hence, we change the structure of \bs, as depicted in Figure~\ref{fig:arch}.

\begin{figure}[h!]
\centering    
\includegraphics[scale=0.35]{Figures/systemModel_BS}
\caption{Internal structure of the proposed Base Station.}\label{fig:arch}
\end{figure}
As shown in Figure \ref{fig:arch}, upon arrival of a task, to a \bs, the \lb~immediately allocates the task either to the receiving \bs~or to a neighboring \bs. A queue is present behind \lb~for the tasks that arrive at the same time. There is no re-allocation considered due to the latency overhead produced by additional task transfer (\ie hops). When the task is allocated to a \bs, it enters batch queue of the \bs~for processing. The time span to complete an arriving task within a \bs~is defined as the \emph{computational delay}. Therefore, $d_\textrm{BS}$ in Equation~\ref{eq:4} is defined as $d_{BS} = d_c$, where $d_c$ is the average computational delay.
\vspace{-2mm}
\subsection{Probability of Meeting Deadline in a Federated V2I System}
The \lb~assigns tasks to the \bs~that offers the highest probability of on-time completion (also defined as \emph{task robustness}). %Calculating the probability of meeting deadline for an arriving task is achieved as follows. 
As shown in Figure~\ref{fig:matrix}, every \bs~maintains two matrices named as Task Completion (ETC) time matrix and Estimated Task Transfer (ETT) time matrix respectively. The ETC Matrix contains estimated task completion time distributions (X$\sim \mathcal{N}(\mu,\,\sigma^{2})$) for different task types in different \bs s. Each ETC matrix entry contains two values, $\mu$ (mean) and $\sigma$ (standard deviation) that are obtained from historical execution time information of each task type on each \bs. We consider that the historic execution time information for each task type on each \bs~form a Normal distribution. In the ETC matrix, every column defines a \bs~and every row defines a task type. 
The Estimated Task Transfer (ETT) time matrix captures the latency of transferring data to another \bs. The entries of ETT are considered as Normal distributions and are obtained from historical data transfer times for different task types from one \bs~to a neighbor. Both ETC and ETT matrices are periodically (\eg approximately every 10 minutes) updated on all \bs s with the help of the central cloud system. 
%The historic transfer time for each task type is shown as Y$\sim \mathcal{N}(\mu,\,\sigma^{2})$).
%To capture the difference between the estimated completion times of task types, we consider the worst-case scenario. Thus, we estimate completion time as the average of the previous completion times summed with its standard deviation. 
%When a vehicle-generated task arrives at the \bs~through the uplink channel, it enters the \lb~where tasks are allocated to appropriate \bs s.

\begin{figure}[h!]
\centering
    \includegraphics[scale=0.35]{Figures/solution.pdf}
    \caption{Proposed allocation model for Load Balancer to efficiently allocate arriving tasks in federated edge computing environment.}\label{fig:matrix}
\end{figure}
%\vspace{-4mm}
Using ETC and ETT matrices, \lb~$j$ that receives task $t_i$ (of task type $i$) can calculate the probability of $t_i$ meeting its deadline $\delta_i$ across all \bs s. For the receiving \bs~$j$, the probability of meeting deadline (denoted as $P_i^j$) is defined based on Equation \ref{eq:6}.
\vspace{-2mm}
\begin{equation}\label{eq:6}
P_i^j (\tau(t_i,bs_j) \ \textless \ \delta_i) \ = \ P_i^j(Z \ \textless \ z)
\end{equation}
In Equation~\ref{eq:6}, $\tau(t_i,bs_j)$ is the expected task completion time. The distribution is standardized with $\mu_i= 0$ and $\sigma_i=1$ using the $z$ score that is formulated based on Equation~\ref{eq:7}.
\vspace{-1mm}
\begin{equation}\label{eq:7}
z = \frac{\delta_i \ - \ \mu_i^j}{\sigma_i^j}
\end{equation}

 
%To obtain the probability, we need to capture the stochasticity that exists both in communication delay and in processing delay. We can leverage distributions available in ETC and ETT matrices for that purpose. More specifically, 

%As we modeled both communication and computation delays in form of Normal distribution, the convolved distribution also has a Normal distribution
To obtain the probability, we convolve the communication and computational delay distributions to find the overall end-to-end delay distribution. This convolved distribution ($W \sim \mathcal{N}(\mu,\ \sigma^{2}) = X \sim \mathcal{N}(\mu,\ \sigma^{2}) \circledast Y \sim \mathcal{N}(\mu \ \sigma^{2}) $) captures the stochasticity that exists both in communication and computation delays. It is worth noting that, our proposed approach is independent from the type of distribution and can be applied on other distributions too. However, as Normal distribution is more general and calculating convolution is faster, we utilize it in this study. %The convolution is defined based on Equation~\ref{eq:8}.
%\vspace{-2mm}
%\begin{equation}\label{eq:8}
%W \sim \mathcal{N}(\mu,\ \sigma^{2}) = X \sim \mathcal{N}(\mu,\ \sigma^{2}) \circledast Y \sim \mathcal{N}(\mu \ \sigma^{2}) 
%\end{equation}
%As we convolve two normal distributions, the resulting distribution is also normal distribution. 
Upon receiving a task by the \lb~$j$, for all of its neighboring \bs s, it convolves the  corresponding entry in the ETC matrix with respective entry in the ETT matrix. 
The resulting distribution for each of the neighboring \bs s is used to calculate the probability of the task meeting its deadline on those \bs s. Once the probability is calculated for all of the \bs s, the arriving task is allocated to the \bs~that offers the highest probability. We note that when the task's probability to meet its deadline is zero, the task is dropped.
%and it will not be allocated to any of the \bs s. 


==> NEW PAPER LATEX/Sources/conclusion.tex <==
\section{Conclusion and Future Works}\label{sec:conclsn}
In this paper, we proposed a robust V2I system that copes with uncertainties that exist in task arrival, communication, and computation. The robustness is provided via federating \bs s in a dynamic manner. The \lb~in each \bs~is equipped with a resource allocation method that is aware of uncertainties in communication and computation of V2I systems.
The uncertainties are captured in a normal distribution and stored in well-defined data structures, known as ETC and ETT matrices. We developed a probabilistic model that predicts the chance of successful completion of a given task on different \bs s that is leveraged in every \lb. The experiments express that the proposed model can significantly improve the robustness of the system (up to 45\%) when it is heavily oversubscribed. It is noteworthy that the system does not only improve the performance of a single \bs~but it also remarkably improves the performance of the V2I system as a whole. In the future, we will extend our probabilistic theory for cases that have heterogeneity within each \bs. We also plan to study the impact of the deadline looseness on the system. 

%From the simulation results, we observed that our proposed heuristic outperforms other heuristics currently used in V2I systems.

%One other avenue of future research is to incorporate the direction of movement of requesting vehicles into the resource allocation process.


==> NEW PAPER LATEX/Sources/experiments.tex <==
\section{Performance Evaluation}\label{experiments}

The most important evaluation metric is considered to be the number of service requests (tasks) that miss their deadline. We evaluate the performance for the system as federation of \bs s, as well as for an individual \bs.

\subsubsection{The Impact of Oversubscription Level}
% In our model, network oversubscription level is said to increase when the number of tasks missing their deadline increases. Therefore, t
To increase the oversubscription level, we increase the number of vehicles that generate service requests, hence, the number of tasks increases. We start initially with 2,000 vehicles passing through the area covered by the network of 15 \bs s in one hour. Each step we increase the traffic by 1,000 vehicles an hour until we reach 7,000 vehicles. In every trial, the simulation is run for 20 times for each one of the state-of-the-art baseline heuristics introduced earlier.

\begin{figure}[h!]
    \centering    
    \includegraphics[scale=0.45]{Figures/overs}
    \caption{Increasing oversubscription level by increasing the number of vehicles served by the network.}
    \label{fig:oversubscriptionLevel}
\end{figure}
%\vspace{-2mm}
%In this experiment, we evaluate the overall performance of the system. That is, the percent of tasks missing their deadlines is calculated with respect to the total number of tasks received by all the \bs s within the system. 
The result of this experiment is shown in Figure~\ref{fig:oversubscriptionLevel}, where the horizontal axis represents the number of vehicles in the system and the vertical axis represents the percent of tasks that missed their deadlines. The number of tasks missing their deadline increases with the higher traffic congestion reflecting the increase in the oversubscription. It also seems reasonable that the No Redirection provides the worst performance compared to all others, as it does not utilizes load balancer.
%have an opportunity to balance the load of service requests. 
The Maximum Certainty heuristic outperforms the MECT at every stage by 1-3\%. Finally, we can observe that BP, consistently outperforms other heuristics (3-8\% better then MECT, 4-11\% better than MC, and  4-17\% better than NR) at every stage of the experiment. We can also notice that it shows the best improvement for medium to high levels of oversubscription (\ie \ 3,000---5,000 vehicles). Additionally, even at an extremely high level of oversubscription (\ie \ 6,000 vehicles), when all other heuristics perform nearly the same, our model still shows improvement, demonstrating its robustness against uncertainty in task arrival intensity. 


\subsubsection{The Impact of Urgency}
To evaluate the performance of our proposed model against the task type arrival uncertainty, we increase the ratio of urgent tasks in the workload from 10\% to 90\% (horizontal axis in Figure~\ref{fig:Urgent}) and account for the number of tasks missing their deadline (vertical axis in Figure~\ref{fig:Urgent}) for every heuristic with high oversubscription (4,000 vehicles) level.
%\vspace{-3mm}
\begin{figure}[h!]
    \centering    
    \includegraphics[scale=0.45]{Figures/ImpactUrgency}
    \caption{The impact of the portion of urgent and non-urgent service requests in the system.}
    \label{fig:Urgent}
\end{figure}
%\vspace{-2mm}
Figure~\ref{fig:Urgent} shows that, deadline miss rate rises, as the percentage of urgent tasks increases. The reason is that urgent tasks have a high delay sensitivity compared to non-urgent tasks. Nevertheless, we can see that our heuristic is robust against task type uncertainties. As the No Redirection shows the poorest performance, with MECT and Maximum Certainty outperforming it by 2-10\%, the Best Probability performs consistently better at all stages of the experiment. When the percentage of urgent tasks is high in the system (70--90\%), the Best Probability outperforms MECT and Maximum Certainty by 5-10\%, as well as the No Redirection by 10-20\%. 
As the percent of urgent tasks begins to dispel, the improvement seems to decrease a little. It is due to the fact that the system becomes less oversubscribed. Thus, we can conclude, that our proposed model offers significant performance improvement when the system is highly congested with delay sensitive tasks. 
%Our proposed system proves to be robust against increased arrival of urgent service requests and can offer an overall better performance when the system is highly congested.

\subsubsection{Single Base Station}
In this experiment, we aim to evaluate the performance of our model with respect to a single \bs~not considering the federation. Just as in the first experiment, we evaluate the system under an increasing oversubscription level of the system as a federation. We start initially with 2,000 vehicles per hour and increase the traffic by 1,000 vehicles until we reach  7,000 vehicles. In every trial, the simulation is run for 20 times for each heuristic. Nevertheless, unlike the first experiment, here we don't account for the overall percent of tasks that miss their deadline within the system. Instead, we evaluate the number of tasks allocated at a certain \bs~that miss their deadline. %Also, a considered \bs~has a three times higher level of oversubscription compared to all neighboring \bs. In other words, as the overall oversubscription level increases, a \bs~under evaluation receives three times as many service requests as the rest of the \bs s in the network.  

%\vspace{-2mm}
\begin{figure}[h!]
    \centering    
    \includegraphics[scale=0.45]{Figures/Single_bs}
    \caption{Average deadline miss rate while increasing the oversubscription level and considering only Base stations that miss the deadlines.}
    \label{fig:networkdelay}
\end{figure}
%\vspace{-2mm}
Figure~\ref{fig:networkdelay} shows a significant performance improvement introduced by our heuristic. The Best Probability performs consistently better then all other heuristics evaluated in the experiment. For the medium level of oversubscription (\ie \ 2,000--3,000 vehicles), Best Probability heuristic shows an improvement of approximately 45\% compared to No Redirection heuristic. Also, it outperforms MECT and Maximum Certainty heuristics by approximately 2-7\% at all stages of the experiment.

%We can conclude that all the experiments demonstrate that our proposed allocation algorithm is more robust than other alternatives. We can observe that Best Probability offers higher robustness at all levels of oversubscription, both in terms of the whole system and a single \bs.



==> NEW PAPER LATEX/Sources/heuristic.tex <==
\section{Resource Allocation Heuristics}\label{sec:heuristcic}
\subsection{Overview}
The following section describes four heuristics considered for the resource allocation. Best Probability is the heuristic we developed based on the proposed model we presented in the previous section. The other two heuristics, Minimum Expected Completion Time, and Maximum Certainty, only utilize the ETC matrix component. Lastly, No Redirection heuristic does not utilize any of the proposed components. 
\vspace{-3mm}
%In fact, the first three heuristics can allocate the arriving requests between all the neighboring \bs s utilizing the edge federation, whereas, the last heuristic is not aware of the edge federation and does not take advantage of the task redirection. It can only allocate arriving tasks to the initial receiving \bs. A more specific description of each heuristic is provided in the following subsections.
\subsection{Best Probability (BP)}
The Best Probability heuristic considers task robustness as the probability of the specific task to meet its deadline in a particular \bs. %For instance, if the probabilities of the task to meet its deadline among 3 base stations ``A," ``B" and ``C" are 0.8, 0.6, 0.5 respectively, then the task has the highest robustness in the \bs~``A."  
As shown in Algorithm~\ref{alg1}, when a \lb~receives a task, it first obtains the task's completion time distribution (using ETC) and the transfer time distribution (using ETT) for the received task type across all the \bs s. Next, it convolves two distributions (except for the receiving \bs, where no transfer will occur) to calculate probabilities for the received task to meet its deadline in all neighboring \bs s. Then, the \lb~chooses the \bs~that provides the maximum value (the highest probability) and allocates the task to that \bs.
%Resulting probabilities are the set of values which represent robustness of the arriving task across the local \bs s. From this robustness set
%For the receiving \bs~the probability is obtained solely from the ETC distribution. 
%Although, the highest probability needs to be greater than zero in order to be allocated. If there is no probability higher than zero within the set than the task is dropped.
%Because only one \bs~can be selected for the allocation, the situation 
When two \bs s have the same highest probabilities, then the tie can be resolved by considering the sparsity (known as standard deviation $\sigma$) of two concurrent distributions. Therefore, the preference is given to the distribution with a smaller standard deviation value.
%The algorithm for the Best Probability heuristic is as follows:

\begin{algorithm}[!h]
	\SetAlgoLined\DontPrintSemicolon
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	\SetKwFunction{algo}{algo}
	\SetKwFunction{proc}{Procedure}{}{}
	\SetKwFunction{main}{\textbf{TaskAssignment}}
	\Input{Task $t_i$; $ETC$ and $ETT$ matrices; $B$ (set of neighboring \bs s)}
	\Output{Chosen \bs~$j\in B$ to assign $t_i$}
    %neiboringBS[] = getNeighborlist(receivingBS)\;
    %bestBS = receivingBS\;
    %deadline = getDeadline(task)\;
    %$P_r$ = getProbabilityETC(receivingBS, task, deadline)\;
    $p_r(t_i) \gets$ Probability on receiving \bs~$r$ \;
    Provisionally assign $t_i$ to receiving \bs~$r$\;
    %$P_{best}$ = $P_r$\;
    \ForEach{\bs~$j \in B$} {
    	%SHOULD WE WRITE ABOUT CONVOLUTION?
    	$p_j(t_i) \gets$ Probability on neighbor edge $j$ \;
    	\If {$p_j(t_i) > p_r(t_i)$} {	%$/* uniqueness$ $dominates$ $on$ $duplicity */$
    		\small{Assign $t_i$ to neighbor \bs~$j$}\;
    		\small{Break}\;
    		%\small{Add $p_j(t_i)$ to $P$, which is  possible edge for assignment}\;
    	}\uElseIf{$p_j(t_i) = p_r(t_i)$}{
    	    
    		\If{$\sigma_j < \sigma_r$}{
    			\small{Assign $t_i$ to neighbor \bs~$j$}\;
    			\small{Break}\;
    			}
        }	
    }
%    \While{ (Traverse neiboringBS list) }{
%        convolvedDistribution  = convolve(ETC, ETT)\;
%        $P_n$ = getProbability(convolvedDistribution,    deadline)\;
%        \uIf{ ($P_n > P_r$)}{
%            bestBS = neiboringBS\;
%            $P_{best}$ = $P_n$\;
%            break\;
%        }
%    \uElseIf{ ($P_n$ == $P_r$) }{
%            $\sigma_r$ = getSigma(receivingBS, task)\;
%            $\sigma_n$ = getSigma(neighboringBS, task)\;
%        \uIf{($\sigma_n > \sigma_r$)}{
%            bestBS = neiboringBS\;
%            $P_{best}$ = $P_n$\;
%                break\;
%        }
%    }
%    }
    \uIf{probability of chosen destination is zero}{
        \small{Drop task $t_i$}\;
    }
        
\caption{Task allocation algorithm for load balancer.}\label{alg1}
\end{algorithm}
\vspace{-4mm}
\subsection{Minimum Expected Completion Time (MECT)}

Minimum Expected Completion Time heuristic is well known and widely described in the recent literatures~\cite{jpdcmohsen,hussain1serverless}. For a received task of a particular type, this heuristic utilizes the ETC matrix to calculate the average expected completion time across all the \bs s and selects the \bs~with minimum expected completion time.

%Its main idea is to find a shortest expected completion time for the received task across all the \bs s and select the \bs with the minimum expected completion time. Hence, this heuristic allocates the tsk to a \bs~which minimizes the expected completion time for a given task type. When the task arrives at the \lb, the ETC matrix is used to calculate the average expected completion time for the task type on every \bs. Then the \lb~selects the \bs~with the shortest expected completion time and allocates the task to that particular \bs. 
\vspace{-3mm}
\subsection{Maximum Certainty (MC)}
Maximum Certainty heuristic (used in~\cite{hussainrobust}) calculates the difference (called certainty ) between the task's deadline and the average completion time for this task type by utilizing ETC matrix. The task is finally assigned to the \bs~that provided the maximum certainty.
\vspace{-2mm}
\subsection{No Redirection (NR)}
No Redirection heuristic does not transfer the task to the neighboring \bs s. Therefore, whenever the arriving task enters the \lb~of a specific \bs, it has to be allocated to that specific \bs. 


==> NEW PAPER LATEX/Sources/relatedwork.tex <==
\section{Related Work}\label{relatedwork}
Efficient resource allocation that can decrease the deadline miss rate is the major challenge for V2I systems. Oversubscription situations make this challenge more complex. The robustness and QoS can deteriorate due to the lack of efficient resource allocation in a V2I system. There are several resource allocation models proposed in the literature. Jun Li et al.\cite{li2017resource} propose a local fog resource management model in Fog Enhanced Radio Access Network based on V2X environment. The core concept is to improve QoS of each \bs~for real-time vehicular services. The model considers service migration from one fog node to another based on reserved resource availability. Authors propose two resource management schemes that prioritize real-time vehicular services. Earlier versions of fog/edge computing were known as hybrid clouds~\cite{salehi10}.

Ali et al. in \cite{ali2011co} propose a multiple RSU (Road Side Unit, e.g., \bs) scheduling to provide cooperative data access to RSUs in vehicular ad-hoc networks. They categorize requests or tasks into two types (delay sensitive and delay tolerant) according to the task's data size.  In oversubscription situations, authors propose to transfer delay tolerant requests to the neighboring RSUs with a lower workload. In contrast we have utilize probabilistic model to find the suitable \bs~that increase the tasks' robustness. In \cite{liu2010rsu}  Liu and Lee suggest an RSU-based data dissemination framework to address challenges in vehicular networks. The system aims to efficiently utilize available bandwidth for both the safety-critical and the non-safety-critical services. An analytical model is proposed to investigate the system performance in terms of providing data services with delay constraints. Adachi et al. in \cite{adachi2016cloud} proposed a hybrid approach, where vehicular content (\eg \ short video clips, sensor data) is shared  among vehicles using V2V and V2I communication via cellular network. The main objective of this paper is to reduce high-cost V2I due to traffic volume in wireless network.

Although various research works have been undertaken in the field of vehicular systems \cite{maeshima2007, korkmaz2006, mak2005}, they are limited to communication functionality, quality requirements from the networking perspective, and task type prioritized scheduling. As compared to the mentioned works, we incorporate both computation and communication aspects to predict the suitable \bs~for task allocation.

%However, none of them considered a V2I system in the aspect of computational capacity and task processing in a \bs~(\eg \ edge device) along with accounting for latency introduced by the networking component. Thus, our work can be distinguished as it contemplates a V2I system in both computational and communicational perspectives.


==> NEW PAPER LATEX/Sources/sec-abs.tex <==
\begin{abstract}
Development of autonomous and self-driving vehicles requires agile and reliable services to manage hazardous road situations. Vehicular Network is the medium that can provide high-quality services for self-driving vehicles. The majority of service requests in Vehicular Networks are delay intolerant (\eg \ hazard alerts, lane change warning) and require immediate service. Therefore, Vehicular Networks, and particularly, Vehicle-to-Infrastructure (V2I) systems must provide a consistent real-time response to autonomous vehicles. During peak hours or disasters, when a surge of requests arrives at a \bs, it is challenging for the V2I system to maintain its performance, which can lead to hazardous consequences. Hence, the goal of this research is to develop a V2I system that is robust against uncertain request arrivals. To achieve this goal, we propose to dynamically allocate service requests among \bs s. We develop an uncertainty-aware resource allocation method for the federated environment that assigns arriving requests to a \bs~so that the likelihood of completing it on-time is maximized. We evaluate the system under various workload conditions and oversubscription levels. Simulation results show that edge federation can improve robustness of the V2I system by reducing the overall service miss rate by up to 45\%.
\end{abstract}

\begin{IEEEkeywords}
Vehicular Networks, Base Station, Vehicle-to-Infrastructure Systems (V2I), Edge Computing, Resource Allocation, Stochastic Model.
\end{IEEEkeywords}



==> NEW PAPER LATEX/Sources/sec-intro.tex <==
\section{Introduction}\label{sec:intro}
Recent advancements in communication and computation technologies have stimulated a rapid development of vehicular networks. Federal Communications Commission (FCC)~\cite{ali2011co} has reserved 5.850 to 5.925 GHz frequency band for Vehicle-to-Everything (\emph{V2X}) communications. Vehicle-to-Infrastructure (V2I) communication is one prominent form of V2X which is visioned under the hood of Intelligent Transport System (ITS) to improve roadside safety and traffic systems. In V2I, infrastructure refers to all the devices (known as Base Stations) that facilitate communications and computations to serve vehicular requests. As shown in Figure~\ref{fig:scen}, autonomous vehicles send their service requests (tasks) to \bs s while operating on the road. A \bs~(BS) is capable of communicating with vehicles and processing vehicular tasks. Examples of such vehicular tasks can be wrong way driver warning~\cite{ABIresearch}, cooperative forward collision warning~\cite{ElBatt}, and lane change warning~\cite{ABIresearch}. This type of tasks can only tolerate a short end-to-end delay, \ie the delay from issuing a task request until receiving its result~\cite{ali2011co}. For such tasks, there is no value in executing them after a tolerable delay.
%, hence, we model an acceptable end-to-end delay as an individual hard deadline for the task. 

%Upon completion of task processing, the results are sent back to the requesting vehicle.
\begin{figure}[h!]
\centering
\includegraphics[scale=0.35]{Figures/scen.jpg}
\caption{A Vehicle to Infrastructure (V2I) scenario where vehicles send requests to a Base Station and receive the response. A Base Station is a roadside unit with communication and computation abilities.\label{fig:scen}}
\end{figure}

%According to literature, V2I systems should incorporate wireless network infrastructure and cloud computing capabilities 
%To enhance the performance of V2I, the Vehicular Cloud Computing (VCC) was initiated in \cite{gerla2012} as a type of Mobile Cloud Computing. However,
Owing to the centralized nature of clouds, both Vehicular Cloud Computing (VCC\cite{gerla2012}) and conventional cloud systems incur high latency~\cite{li2017resource}. Nonetheless, \bs's computational power can be harnessed with an edge computing system that can manage vehicular services at the \bs~with low latency without communicating to cloud datacenter. Various \bs s in a V2I system can potentially be heterogeneous, both in terms of computational characteristics and communication medium to the core network (\eg wireless, optical, and wired).
%With the edge device, vehicular services can be managed directly at the \bs~with low latency without  
%~\cite{bok2016multiple}
%and cannot be used for delay intolerant tasks.
A problem arises during road emergencies (\eg road accidents or disasters) when a rapid increase in service requests to \bs s significantly affects the tasks' service time. In fact, in this situation, \bs~resources become oversubscribed, and many tasks miss their deadlines due to insufficient computational resources.
%it cannot provide enough computational power for all the arriving tasks to meet their deadlines. 
%Such circumstance in a V2I system can potentially cause fatal damage to vehicles and/or people.

\emph{Robustness} is defined as the degree to which a V2I system can maintain a certain level of performance even in the presence of stochastic parameters in the system~\cite{jpdcmohsen,li2017cost,ali2004measuring}. Accordingly, our goal, in this research, is to design a V2I system that is robust against uncertain task arrival. In this research, we evaluate robustness of the V2I system according to the number of tasks that can meet their deadlines. The main question we try to answer is stated as how to allocate arriving tasks among the \bs s so, the systems' robustness is maximized? An efficient solution to this problem needs to overcome the uncertainties (\eg uncertain task arrival, task execution times, communication delay) of the system. 
%In particular, uncertainties introduced by uncertain task arrival, task execution times, and communication delay. 
%For that purpose, tasks should be allocated so that the number of tasks meeting their deadlines is maximized.
Previous research works either discard these uncertainties\cite{bok2016multiple} or focus only on one of the aforementioned uncertainty factors (\eg communication\cite{ali2011co}). Alternatively, we propose a robust model that copes with uncertainties introduced by the task arrival, communication, and computation. To cope with the uncertainty in task arrival, we propose to federate \bs s and devise a \lb~at the \bs~that can leverage the computational capabilities of neighboring \bs s to improve robustness of the V2I system. 
%to assure robustness of the V2I system,
%Then, we develop a probabilistic theory that can capture the uncertainties in the federated environment.

%To cope with the uncertainties in communication and computation,

Allocating vehicular tasks in a V2I system is proven to be an NP-complete problem~\cite{Ullman1975}. Therefore, a large body of research works have been dedicated to developing resource allocation heuristics in such systems~\cite{ali2004measuring,yu2016optimal,li2017resource,liu2010rsu}. As such, we leverage our proposed probabilistic theory and establish a novel resource allocation heuristic for the \bs s' \lb. Then, we evaluate the performance of our proposed heuristic under various workload conditions.
%The resource allocation method is deployed within the load balancer of the federated \bs s (\ie edge nodes).
%Lenstra1981, pyun2016,
The main contributions of this paper are as follows:

\begin{itemize}
    \item Propose a system that encompasses the uncertainties that exist in task arrival, communication, and computation.
    \item Devise a probabilistic theory to predict the success of task completion within the deadline on different \bs s.
    \item Develop a load balancing heuristic that functions based on the proposed theory and increases the robustness of the V2I system.
    \item Analyze the performance of our proposed system under various workload conditions and in comparison to different existing models.
\end{itemize}

The rest of the paper is organized as follows. Section \ref{sec:scen} introduces the System Model and Problem Statement. Section \ref{sec:approach} discusses the robust V2I system based on federated \bs s. Sections \ref{sec:heuristcic} and \ref{sec:simulation} present resource allocation heuristics and experimental setup respectively. Performance evaluation is presented in section \ref{experiments}. Section \ref{relatedwork} presents Related Work. Finally, section \ref{sec:conclsn} concludes the paper.% with some future directions.


==> NEW PAPER LATEX/Sources/sec-scen.tex <==
\section{System Model and Problem Statement}\label{sec:scen}
\subsubsection{Scenario}
%This research is motivated by a V2I system in which vehicles issue service requests (tasks) while traveling through roads, highways, and intersections. Once a task is issued, it is sent to the Road Side Unit for processing. Finally, the results are returned to the issuing vehicle upon processing completion.

The Road Side Unit, or as we call it, a \bs~is located at the intersection or the side of the road. \bs s are stationary edge devices with memory, storage, computational ability, and short wireless range transmission system \cite{liu2010rsu}. The receiving \bs~is connected to a number of nearby heterogeneous \bs~via 5G wireless network~\cite{yu2016optimal}. In summary, the receiving \bs~can transfer tasks to the neighboring \bs s, that forms a federation of \bs s. Every \bs~in the federation is also connected to a central cloud infrastructure. In this scenario, the roads and intersections are considered to be congested. Therefore, the \bs~situated at the roadsides and intersections is oversubscribed. %(\ie it is not capable of serving all the incoming requests).  
%That is, we observe only medium to high levels of traffic jams
In our scenario, all tasks have an individual deadline, the time frame in which tasks should be processed and returned to the vehicle. Based on the specific service required, tasks are separated into two groups, urgent (delay-intolerant) and non-urgent (delay-tolerant). For example, Hazards Around the Area alerts are considered to be urgent, and the On-board Entertainment updates are considered non-urgent. According to the task type, non-urgent tasks usually are bigger in data size and need more time to execute. Respectively, urgent tasks are smaller in data size. 
%In our scenario, the execution of the task that has missed its deadline has no value. For instance, consider a vehicle requesting an update on the road conditions of a specific street. If there is no response by the time the vehicle has reached to the street, there is no value to the requested update.

%By considering the above-mentioned scenario, the specific research problem is stated as \textit{how to allocate arriving tasks along the \bs s in a V2I network so that the number of tasks missing their deadline is minimized?}

\subsubsection{Assumptions}
According to the described scenario, a set of tasks is generated by vehicles and sent to the \bs~for processing. Every task $i$ has its own deadline (denoted $\delta_i$) within which it has to be completed. The V2I system allocates the tasks to \bs s by considering the individual deadline for each task. 
To enable robustness, the resource allocation method aims to maximize the number of tasks meeting their deadlines. 

According to the problem definition, the set of arriving tasks can be defined as $T$, where  $T$ = $\{t_1, t_2, t_3, t_4\dots, t_n\}$ and the set of Base Stations defined as $BS$, where $BS$ = $\{bs_1, bs_2, bs_3, bs_4\dots, bs_m\}$. The set of tasks that can meet their deadlines, denoted $T_s$, is the subset of $T$ ($T_s \subseteq T$).

%We define Bernoulli random variable $\kappa$, such that:

%\begin{equation}\label{eq:1}
%    \kappa(t_i,bs_j) \ = \
%    \left\{
%        \begin{array}{cc}
%  
%       1 \ \ \ \ if \ \tau(t_i,bs_j)\leq \delta_i \\
%       0 \ \ \ \ \ \ \ \ \ \ \ \mathrm{otherwise}\\
%        
%        \end{array}   
%    \right.
%\end{equation}
%
%%where $\delta_i$ is the deadline for task type $i$. 
%That is, $\kappa(t_i,bs_j)$ is equal to 1, if task $t_i$ is completed before $\delta_i$ at a \bs~$j$ (\ie $\tau(t_i,bs_j)\leq \delta_i$), otherwise, $\kappa(t_i,bs_j)$ is equal to 0. It is assumed that task $t_i$ is allocated to the base station $bs_j$ when the task $t_i$ is projected to meet its deadline $\delta_i$ in that specific base station $bs_j$. 

%Therefore, the problem can be formulated as:

%\begin{equation}\label{eq:2}
%\begin{aligned}
%&  \underset{\tau}{\text{maximize}}
%& & \sum_{i=1}^{n} \sum_{j=1}^{m} \tau(t_i,bs_j), \ where \ t_i \in T_s \ and \ bs_j \in BS\\
%& \text{subject to}
%& &  t_i \leq \delta_i\;
%\end{aligned}
%\end{equation}



Upon arrival to a \bs, the task is assigned an individual deadline that includes task arrival time and the end-to-end delay the task can tolerate. We assume in our case that communication delay (uplink and downlink delay) can be significant. Thus, we consider a communication delay for a deadline calculation as well. For arriving task $t_i$, the deadline is defined based on Equation~\eqref{eq:2}.
\vspace{-2mm}
\begin{equation}\label{eq:2} 
\delta_i = arr_i + E_i + \epsilon + \beta 
\end{equation} 

where $arr_\textrm{i}$ is the arrival time of the task, $E_\textrm{i}$ is the average task completion time, $\epsilon$ is a constant value defined by the \bs~(slack time), and $\beta$ is the communication delay. We assume that tasks arrive at the \bs~dynamically, and the arrival rate is not known in advance. As we consider, receiving \bs~is oversubscribed, therefore, some tasks are projected to miss their deadline. If such tasks are delay-sensitive, then they are dropped, which is a common practice in oversubscribed real-time systems \cite{jpdcmohsen}.

%In this research, we define the tasks' robustness as its probability to meet the deadline in a particular \bs. For example, if an arriving task has a greater probability to meet its deadline in Base Station $A$ among a cluster of \bs s, then \bs~$A$ provides greater robustness for this task.

% Also, even though it is mentioned that all the Base Stations of the local network are connected to the cloud server, we are not considering cloud server for task processing due to its significant communication latency.

\subsubsection{Delay Estimation}
In a V2I system, three distinct factors contribute to the end-to-end delay. They are uplink delay, computational delay, and downlink delay~\cite{mostafa2011}. Therefore, V2I end-to-end delay (denoted $D_\textrm{V2I}$) is defined based on Equation~\eqref{eq:3}. 
\vspace{-2mm}
\begin{equation}\label{eq:3}
D_\textrm{V2I} = d_\textrm{U} + d_\textrm{BS} + d_\textrm{D} 
\end{equation} 

where $d_U$ is average uplink delay, $d_\textrm{BS}$ is average computational delay, and $d_D$ is average downlink delay. 

From Equation \eqref{eq:3}, $d_U$  and $d_D$ can be defined as follows. For task $i$  requested by the vehicle $v$ to the \bs~$m$, the uplink delay from $v$ to $m$ is defined based on Equation~\eqref{eq:4}.
\vspace{-2mm}
\begin{equation}\label{eq:4} 
d_\textrm{U} =  \frac{L_\textrm{i}}{g(v,m)}  
\end{equation} 

and for $t_i$ traveling back from the \bs~$m$ to a vehicle $v$, the downlink delay is defined based on Equation~\eqref{eq:5}.
\vspace{-2mm}
\begin{equation}\label{eq:5} 
d_\textrm{D} =  \frac{L_\textrm{i}}{g(m,v)} 
\end{equation} 

where $L_i$  is the task data size, $g(v,m)$ and $g(m,v)$ is bandwidth for the link from $v$ to $m$ and from $m$ to $v$, respectively.


%\subsubsection{\textbf{System Model}}
% Upon the arrival to the \bs~the task gets into the \lb~component. \lb~allocates the service request immediately upon arrival. A queue is present in every \lb~for the tasks that arrive at the same time. There is no re-allocation considered after the task has been allocated by the \lb~due to the overhead produced by additional task transfer. \lb~can allocate the task to the receiving \bs~or to any of the neighboring \bs s. When the task is allocated, it enters the batch queue of the \bs~for processing. From the arrival to the end of the task, a processing delay is imposed. Such a delay can be defined as a \emph{computational delay} (denoted $d_c$). Therefore, $d_\textrm{BS}$ can be defined as $d_{BS} = d_c$, where $d_c$ is an average computational delay.


==> NEW PAPER LATEX/Sources/sec-sysmodel.tex <==

\section{System Model}

  


==> NEW PAPER LATEX/Sources/simulation.tex <==
\section{Experimental Setup}\label{sec:simulation}
We have used EdgeCloudSim~\cite{sonmez2017edgecloudsim}, a discrete edge simulator to evaluate the performance of our proposed model. Due to computational resource limitation, we implement \bs s in a form of small data centers, with up to 4 cores having computational capacity of 1600 Million Instructions Per Second (MIPS) for each core. All Virtual Machines (VMs) in a \bs~are homogeneous, \ie~same computational power. Nevertheless, \bs s are heterogeneous \ie~have different computational powers. In simulation, we have a total of 15 \bs s, where 8 of them are the 4-core \bs s and 7 are the 2-core \bs s. Each \bs~in has a specified location in an X-Y plane, which is utilized by the Mobility model of EdgeCloudSim to find the closest \bs~to a simulated vehicle. 
%In vehicular networks, there are two types of \bs s, the bigger ones with 4 cores and the smaller ones with 2 cores.
%Each core is utilized by one Virtual Machine (VM)
%Each \bs~also has an attraction level that demonstrates its potential of being utilized. By default, we use the same attraction level for all the \bs s.
We also utilize 4 types of tasks in our simulation where 2 of those types are urgent and the other 2 are non-urgent. Specifically, we implement a Hazard Alert and the Lane Change Warning as the urgent task types (2000-3000 MIPS). The other two types are the On-Board Entertainment and the Fuel Usage Statistics (10000-15000 MIPS).

For the networking model, we specify the Wireless Local Area Bandwidth (WLAN) with 200 MBps. This delay is imposed only when the \lb~transfers tasks to a neighboring \bs~(known as LAN delay) is set to be 2 seconds. By default, the requests are initially offloaded to the nearest \bs, and only then, the load balancer assign receiving task to suitable \bs.
%load balanced, as every \bs~in our simulation possesses a load balancing component. 
For the workload generation, the tasks are sampled randomly from the Exponential distribution. Each \bs~receives a certain amount of service requests as a receiving \bs, as well as the certain amount of tasks, transferred from the neighboring \bs s. We consider maintaining ETC and ETT matrices in every \bs~and update them in every 10\% of the workload execution. The workloads are seeded and changed from one trial to another.

%The Mobility model provided by the EdgeCloudSim is utilized to create positions for the vehicles in the X-Y plane.
 
%we used EdgeCloudSim workload generator, known as Scenario Factory. 

%We used Louisiana Optical Network Infrastructure (LONI)~\cite{LONI}, which is the most powerful supercomputer in Louisiana for performing research and industrial activities.

     


==> Sources/sec-sysmodel.tex <==

\section{System Model}

  

